Human-Machine Collaboration for Democratizing Data Science

Everybody wants to analyse their data, but only few posses the data science expertise to to this. Motivated by this observation we introduce a novel framework and system \textsc{VisualSynth} for human-machine collaboration in data science. It wants to democratize data science by allowing users to interact with standard spreadsheet software in order to perform and automate various data analysis tasks ranging from data wrangling, data selection, clustering, constraint learning, predictive modeling and auto-completion. \textsc{VisualSynth} relies on the user providing colored sketches, i.e., coloring parts of the spreadsheet, to partially specify data science tasks, which are then determined and executed using artificial intelligence techniques.

==> sections/synthlog.tex <==
\section{SynthLog, a language for data science}

\clement{Put synthlog as related work?}

SynthLog is a language for supporting automated data science processes. It allows to construct and manipulate inductive data models.
An {\em Inductive Data Model (IDM)} consists of 1) a set of data models (DM) that specifies an adequate data structure for the dataset (like a database), and 2) a set of inductive models (IMs), that is, a set of patterns and machine learning models (like classifiers) that have been discovered in the data. While the DM can be used to retrieve information about the dataset and to answer questions about specific data points, the IMs can be used to make predictions, find inconsistencies and redundancies, etc.
IDMs integrate data and inductive models in a SynthLog {\em theory}.
 
SynthLog is built on top of the ProbLog probabilistic programming language. It essentially assumes that both the data models and the inductive models are ProbLog programs, and allows to refer to and manipulate such models by means of a new ProbLog operator. Building on top of Probabilistic Logic Programming is a key feature of SynthLog. Indeed, a key challenge of designing systems that interact with users is the fact that they can be imprecise and inconsistent. As probabilistic reasoning is a way to deal with uncertainty, SynthLog is well suited to be the back-end of systems interacting with end-users.

As SynthLog manipulates both data and inductive models, it borrows ideas from inductive databases that also consider both data and inductive models as first class citizens. For example, SynthLog follows the mantra of inductive databases that requires the closure property to be satisfied \cite{imielinski1996database,de2002perspective}. In the SynthLog context this means that the result of any operation must be a theory, and thus must be a ProbLog program. At the same time, as each theory is a ProbLog program, SynthLog supports deductive and probabilistic reasoning, a form of answer set programming (through DTProbLog \cite{van2010dtProbLog}) and machine learning.

Well known tools such as auto-sklearn \cite{feurer2015efficient} or auto-Weka \cite{thornton2013auto} are automating Machine Learning, and some of the associated preprocessing. SynthLog differs from this tools because it is automating Data Science. Hence, SynthLog supports many Data Science tasks -- and Machine Learning is one of these tasks -- and is suited to interact with users, as SynthLog can handle rules and constraints, that are a typical way of adding user knowledge in the learning process.
\clement{See how much deeper we should go into explaining SynthLog}
